A Spectroscopic Survey of the Fields of 28 Strong Gravitational Lenses: Implications for $H_0$

Strong gravitational lensing provides an independent measurement of the Hubble parameter ($H_0$). One remaining systematic is a bias from the additional mass due to a galaxy group at the lens redshift or along the sightline. We quantify this bias for more than 20 strong lenses that have well-sampled sightline mass distributions, focusing on the convergence $\kappa$ and shear $\gamma$. In 23% of these fields, a lens group contributes a $\ge$1% convergence bias; in 57%, there is a similarly significant line-of-sight group. For the nine time delay lens systems, $H_0$ is overestimated by 11$^{+3}_{-2}$% on average when groups are ignored. In 67% of fields with total $\kappa \ge$ 0.01, line-of-sight groups contribute $\gtrsim 2\times$ more convergence than do lens groups, indicating that the lens group is not the only important mass. Lens environment affects the ratio of four (quad) to two (double) image systems; all seven quads have lens groups while only three of 10 doubles do, and the highest convergences due to lens groups are in quads. We calibrate the $\gamma$-$\kappa$ relation: $\log(\kappa_{\rm{tot}}) = (1.94 \pm 0.34) \log(\gamma_{\rm{tot}}) + (1.31 \pm 0.49)$ with a rms scatter of 0.34 dex. Shear, which, unlike convergence, can be measured directly from lensed images, can be a poor predictor of $\kappa$; for 19% of our fields, $\kappa$ is $\gtrsim 2\gamma$. Thus, accurate cosmology using strong gravitational lenses requires precise measurement and correction for all significant structures in each lens field.

==> revtex4-1/00readme.tex <==
\title{%
 The \classname{revtex4-1} document class of the American Physical Society%
 \protect\thanks{Work under hire to The American Physical Society.}%
}%
\author{Arthur Ogawa%
 \protect\thanks{First revision of REV\TeX4.0 (unreleased) by David Carlisle}%
}%
\date{Version \fileversion, dated \filedate}%
\newcommand\revtex{REV\TeX}

\maketitle

This file embodies the implementation of the APS \revtex\ 4.1 document class
for electronic submissions to journals.

The distribution point for this work is
\url{http://publish.aps.org/revtex4/},
which contains fully unpacked, prebuilt runtime files and documentation.

\tableofcontents

\section{Using \protect\revtex}

The file \file{README} has retrieval and installation information.

User documentation is presented separately in \file{auguide.tex}.

The file \file{template.aps} is a boilerplate file.

\changes{4.0a}{1998/01/16}{Initial version}
\changes{4.0a}{1998/01/31}{Move after process options, so \cs{clearpage} not in scope of twocolumn}
\changes{4.0a}{1998/01/31}{Rearrange the ordering so numerical ones come first. AO: David, what does this mean?}
\changes{4.0a}{1998/01/31}{use font-dependent spacing}
\changes{4.0a}{1998/01/31}{4.0d had twoside option setting twoside switch to false}
\changes{4.0a}{1998/01/31}{Move after process options, so the following test works}
\changes{4.0a}{1998/01/31}{print homepage}
\changes{4.0a}{1998/01/31}{protect against hyperref revtex kludges which are not needed now}
\changes{4.0a}{1998/06/10}{multiple preprint commands}
\changes{4.0a}{1998/06/10}{comma not space between email and homepage}
\changes{4.0a}{1998/06/10}{single space footnotes}
\changes{4.0b}{1999/06/20}{First modifications by Arthur Ogawa (mailto:arthur\_ogawa at sbcglobal dot net)}
\changes{4.0b}{1999/06/20}{Added localization of \cs{figuresname}}
\changes{4.0b}{1999/06/20}{Added localization of \cs{tablesname}}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{10pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{11pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{12pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: made aps.rtx part of revtex4.dtx}
\changes{4.0b}{1999/06/20}{AO: remove duplicates}
\changes{4.0b}{1999/06/20}{call \cs{print@floats}}
\changes{4.0b}{1999/06/20}{Defer assignment until \cs{AtBeginDocument} time.}
\changes{4.0b}{1999/06/20}{Defer decision until \cs{AtBeginDocument} time}
\changes{4.0b}{1999/06/20}{Define three separate environments, defer assignment to \cs{AtBeginDocument} time.}
\changes{4.0b}{1999/06/20}{Frank Mittelbach, has stated in \protect\classname{multicol}: ``The kernel command \cs{@footnotetext} should not be modified.'' Thus, I have removed David Carlisle's redefinition of that command. Note, however, that later versions of \protect\classname{multicol} do not require this workaround. Belt and suspenders.}%
\changes{4.0b}{1999/06/20}{Move this ``complex'' option to the front, where it can be overridden by ``simple'' options.}
\changes{4.0b}{1999/06/20}{New option}
\changes{4.0b}{1999/06/20}{One-line caption sets flush left.}
\changes{4.0b}{1999/06/20}{only execute if appropriate}
\changes{4.0b}{1999/06/20}{Processing delayed to \cs{AtBeginDocument} time}
\changes{4.0b}{1999/06/20}{Removed invocation of nonexistent class option \protect\classoption{groupauthors} and all other class options that should only be invoked by the document. (Otherwise precedence of class options does not work.)}
\changes{4.0b}{1999/06/20}{Restore all media size class option of \protect\file{classes.dtx}}
\changes{4.0b}{1999/06/20}{Stack \cs{preprint} args flush right at right margin.}
\changes{4.0c}{1999/11/13}{(AO, 115) If three or more preprints specified, set on single line, with commas.}
\changes{4.0c}{1999/11/13}{(AO, 129) section* within appendix was producing appendixname}
\changes{4.0c}{1999/11/13}{*-form mandates pagebreak}
\changes{4.0c}{1999/11/13}{also spelled ``acknowledgements''.}
\changes{4.0c}{1999/11/13}{Do not put by REVTeX in every page foot}
\changes{4.0c}{1999/11/13}{grid changes via ltxgrid procedures}
\changes{4.0c}{1999/11/13}{grid changes with ltxgrid}
\changes{4.0c}{1999/11/13}{Insert procedure \cs{checkindate}}
\changes{4.0c}{1999/11/13}{Lose compatability mode.}
\changes{4.0c}{1999/11/13}{New ltxgrid-based  code, other bug fixes}
\changes{4.0c}{1999/11/13}{New option ``checkin''}
\changes{4.0c}{1999/11/13}{Prevent an inner footnote from performing twice}
\changes{4.0d}{2000/04/10}{Also alter how lists get indented.}
\changes{4.0d}{2000/04/10}{eprint takes an optional argument, syntactical only in this case.}
\changes{4.0d}{2000/04/10}{New option}
\changes{4.0d}{2000/05/10}{More features and bug fixes: compatability with longtable and array packages. Now certainly incompatible with multicol.}
\changes{4.0d}{2000/05/17}{make longtable trigger the head, too}
\changes{4.0d}{2000/05/18}{But alternative spelling is deprecated.}
\changes{4.0e}{2000/09/20}{New option showkeys}
\changes{4.0e}{2000/11/14}{Bug fixes and minor new features: title block affiliations can have ancillary data, just like authors; clearpage processing revamped, with floats staying in order; widetext ornaments.}
\changes{4.0e}{2000/11/21}{adornments above and below.}
\changes{4.0f}{2001/02/13}{Last bug fixes before release.}
\changes{4.0rc1}{2001/06/17}{Running headers always as if two-sided}
\changes{4.0rc1}{2001/06/18}{grid changes with push and pop}
\changes{4.0rc1}{2001/06/18}{grid changes with push and pop}
\changes{4.0rc4}{2001/07/23}{hyperref is no longer loaded via class option: use a usepackage statement instead}
\changes{4.1a}{2008/01/18}{(AO, 457) Endnotes to be sorted in with numerical citations.}%
\changes{4.1a}{2008/01/18}{(AO, 451) ``Cannot have more than 256 cites in a document''}%
\changes{4.1a}{2008/01/18}{(AO, 457) Endnotes to be sorted in with numerical citations.}%
\changes{4.1a}{2008/01/18}{(AO, 460) ``Proper style is "FIG. 1. ..." (no colon)''}%
\changes{4.1a}{2008/01/18}{(AO, 478) \cs{ds@letterpaper}, so that ``letterpaper really is the default''}%
\changes{4.1a}{2008/01/18}{(AO, 488) Change processing of options to allow an unused option to specify society and journal}%
\changes{4.1a}{2008/01/19}{(AO, 461) Change the csname revtex uses from @dotsep to ltxu@dotsep. The former is understood in mu. (What we wanted was a dimension.)}%
\changes{4.1a}{2008/01/19}{For natbib versions before 8.21, \cs{NAT@sort} was consulted only as natbib was being read in. Now it is fully dynamic.}
\changes{4.1b}{2008/05/29}{The csname substyle@ext is now defined without a dot (.), to be compatible with \LaTeX usage (see @clsextension and @pkgextension).}
\changes{4.1b}{2008/06/01}{(AO) Implement bibnotes through \cs{frontmatter@footnote@produce} instead of \cs{bibnotes@sw}}%
\changes{4.1b}{2008/06/01}{Add option reprint, opposite of preprint, and preferred alternative to twocolumn}
\changes{4.1b}{2008/06/29}{(AO, 455) Be nice to a list within the abstract (assign \cs{@totalleftmargin}).}
\changes{4.1b}{2008/06/30}{(AO) Structure the Abstract using the \texttt{bibliography} environment}
\changes{4.1b}{2008/07/01}{(AO) coordinate \cs{if@twoside} with \cs{twoside@sw}}
\changes{4.1b}{2008/07/01}{(AO) make settings at class time instead of deferring them to later.}
\changes{4.1b}{2008/07/01}{(AO) No longer need to test \cs{chapter} as of \texttt{natbib} version 8.2}
\changes{4.1b}{2008/07/01}{(AO) No longer use \cs{secnumarabic@sw}, instead use \cs{setup@secnums}}
\changes{4.1b}{2008/07/01}{(AO) Provide more diagnostics when \cs{@society} is assigned.}
\changes{4.1b}{2008/07/01}{(AO) provide option longbibliography}
\changes{4.1b}{2008/07/01}{Add \cs{@hangfroms@section}}
\changes{4.1b}{2008/07/01}{Break out \cs{@caption@fignum@sep}}
\changes{4.1b}{2008/07/01}{Class option galley sets \cs{preprintsty@sw} to false}
\changes{4.1b}{2008/07/01}{Code relating to new syntax for frontmatter has been placed in \file{ltxfront.dtx}}
\changes{4.1b}{2008/07/01}{Package textcase is now simply a required package}
\changes{4.1b}{2008/07/01}{Procedures \cs{@parse@class@options@society} and \cs{@parse@class@options@journal} and friends}
\changes{4.1b}{2008/07/01}{Read in all required packages together}
\changes{4.1b}{2008/07/01}{Remove options newabstract and oldabstract}
\changes{4.1b}{2008/08/01}{Section numbering via procedures \cs{secnums@rtx} and \cs{secnums@arabic}.}
\changes{4.1b}{2008/08/04}{As with author formatting, rag the right more, and assign \cs{@totalleftmargin}. Also neutralize \cs{def@after@address}.}%
\changes{4.1b}{2008/08/04}{Rag the right even more: .8\cs{hsize}. Also, assign \cs{@totalleftmargin}.}%
\changes{4.1b}{2008/08/04}{The \texttt{rmp} journal substyle selects \texttt{groupedaddress} by default.}%
\changes{4.1b}{2008/08/04}{Use \cs{setup@hook} to initialize all.}
\changes{4.1c}{2008/08/15}{Document class option longbibliography via \cs{substyle@post}}
\changes{4.1d}{2009/03/27}{Definition of \cs{ @fnsymbol} follows fixltx2e.sty}
\changes{4.1e}{2008/06/29}{(AO, 455) be nice to a list within the abstract}
\changes{4.1f}{2009/07/07}{(AO, 513) Add class option linenumbers: number the lines a la \classname{lineno}}
\changes{4.1f}{2009/07/07}{(AO, 516) Merged references are separated with a semicolon}
\changes{4.1f}{2009/07/10}{(AO, 520) Automatically produce \cs{bibliography} command when needed}%
\changes{4.1f}{2009/07/11}{(AO, 521) Lonely bibliography head}%
\changes{4.1f}{2009/07/11}{(AO, 522) Warn if software is expired}%
\changes{4.1f}{2009/07/15}{(AO, 523) Add class option nomerge, to turn off new natbib 8.3 syntax}
\changes{4.1f}{2009/07/20}{(AO, 524) Makes no sense if citations are superscript numbers and so are footnotes}
\changes{4.1f}{2009/10/05}{(AO, 530) \cs{@fnsymbol}: Failed to import fixltx2e.sty technology. Return to LaTeX core.}
\changes{4.1g}{2009/10/07}{(AO, 525) Remove phantom paragraph above display math that is given in vertical mode}%
\changes{4.1g}{2009/10/07}{(AO, 538) \cs{MakeTextUppercase} inappropriately expands the double backslash}
\changes{4.1h}{2009/10/09}{(AO) Remove expiry code in the release software}%
\changes{4.1i}{2009/10/23}{(AO, 541) Defer assignment of \cs{cite} until after natbib loads}
\changes{4.1j}{2009/10/24}{(AO, 549) Repairing natbib's \cs{BibitemShut} and \cs{bibAnnote}}
\changes{4.1j}{2009/10/25}{(AO, 545) hypertext capabilities off by default; enable with \classoption{hypertext}}
\changes{4.1j}{2009/10/25}{(AO, 552) Repair spacing in \cs{onlinecite}}
\changes{4.1k}{2009/11/06}{(AO, 554) give the \cs{newlabel} command syntax appropriate to the hyperref package}
\changes{4.1n}{2009/11/06}{(AO, 565) restore 4.0 behavior: invoking class option preprint implies class option preprintnumbers}
\changes{4.1n}{2009/11/30}{(AO, 566) restore 4.0 behavior: flush column bottoms}
\changes{4.1n}{2009/12/05}{(AO, 569) Use of \classname{hyperref} interferes with column balancing of last page}%
\changes{4.1n}{2009/12/09}{(AO, 569) execute the after-last-shipout procedures from within the safety of the output routine}%
\changes{4.1n}{2010/01/02}{(AO, 571) Interface \cs{set@footnotewidth} for determining the set width of footnotes}%
\changes{4.1n}{2010/01/02}{(AO, 572) Independent footnote counter for title block. Abstract footnote counter shared with body.}%
\changes{4.1n}{2009/12/13}{(AO, 573) arrange to load \classname{lineno} after any other packages.}%
\changes{4.1n}{2010/01/04}{(AO, 575) the default for journal prstper is longbibliography}%
\changes{4.1n}{2010/01/04}{(AO, 576) In .bst files, remove support for the annote field}%
\changes{4.1n}{2010/01/02}{(AO) fine-tune spacing above and below widetext}%
\changes{4.1n}{2010/01/02}{(AO, 571) class file must set \cs{splittopskip}; fine tune \cs{skip}\cs{footins}; \cs{footnoterule} defined in terms of \cs{skip}\cs{footins}}%
\changes{4.1n}{2010/01/02}{(AO, 572) \cs{@makefntext} and \cs{frontmatter@makefntext} must be defined harmoniously}%
\changes{4.1o}{2010/02/02}{(AO, 575) Automatically incorporate the (Bib\TeX-generated) .bbl into an explicit \env{thebibliography}}%
\changes{4.1o}{2010/02/05}{(AO, 549) Remove patch to natbib, which is now at version 8.31a}
\changes{4.1o}{2010/02/07}{(AO, 578) accommodate the possible space character preceding \cs{BibitemShut}.}
\changes{4.1o}{2010/02/05}{(AO, 579) Endnote shall comprise their own Bib\TeX\ entry type: @FOOTNOTE.}
\changes{4.1o}{2010/02/10}{(AO, 580) Provide a document class option to turn off production of eprint field in bibliography.}
\changes{4.1o}{2010/02/12}{(AO, 580) Control .bst at run time.}%
\changes{4.1o}{2010/02/09}{(AO, 581) Handle case: merged references, with first ending in a stop character.}
\changes{4.1p}{2010/02/24}{(AO, 583) Provide interface to \classname{ltxgrid} \cs{onecolumn@grid@setup} and \cs{twocolumn@grid@setup}}
\changes{4.1p}{2010/02/24}{(AO, 584) Per MD, remove trailing space character from each journal abbreviation: it had caused an extraneous space in the .bbl}
\changes{4.1q}{2010/04/01}{(AO, 586) When .bbl is pasted into the document, prevent automatic bibliography inclusion.}%
\changes{4.1q}{2010/04/13}{(AO, 588) Only write \revtex-specific BibTeX .bib data if the .bst style is set by REVTeX.}%
\changes{4.1r}{2010/06/22}{(AO, 595) Provide \cs{lovname} along with other List of Videos definitions.}%

\iffalse ltxdoc klootch
This file has version number 4.1r, last revised 2010/07/25/20:33:00.\fi


==> revtex4-1/README <==
%% ****** Start of file README ****** %
%%
%%   This file is part of the APS files in the REVTeX 4 distribution.
%%   Version 4.1r of REVTeX, August 2010.
%%
%%   Copyright (c) 1999, 2000, 2001, 2009, 2010 The American Physical Society.
%%

Last updated 09 August 2010

This file describes the contents of this distribution of REVTeX 4.1.
The definitive source of information about REVTeX 4 is the APS web
page http://authors.aps.org/revtex4/.

User queries should be directed to revtex@aps.org.

Manifest
--------

All files in this release are contained within the compressed archive
revtex4-1.zip. For installation instructions, see below.

NOTE: The only files necessary for running REVTeX 4.1 are those under 
tex/latex/revtex and bibtex/bst/revtex, but it is a good idea to install
the entire distribution, especially the documentation.

TeX inputs:          tex/latex/revtex/
                     -----------------  
revtex4-1.cls     - The REVTeX 4.1 class file
aps4-1.rtx        - APS-specific customizations for REVTeX 4.1
aip4-1.rtx        - AIP-specific customizations for REVTeX 4.1
apsrmp4-1.rtx     - APS-specific customizations for REVTeX 4.1,
                    specifically for Rev. Mod. Phys.
aps10pt4-1.rtx    - 10-point size class option file for REVTeX.
aps11pt4-1.rtx    - 11-point size class option file for REVTeX.
aps12pt4-1.rtx    - 12-point size class option file for REVTeX.
revsymb4-1.sty    - A collection of common symbols for use outside of REVTeX.

ltxdocext.sty     - Part of ltxgrid package used for page layout in REVTeX.
ltxfront.sty      - Part of ltxgrid package used for page layout in REVTeX.
ltxgrid.sty       - Part of ltxgrid package used for page layout in REVTeX.
ltxutil.sty       - Part of ltxgrid package used for page layout in REVTeX.
  
BibTeX inputs:       bibtex/bst/revtex/
                     ------------------ 
apsrev4-1.bst     - BibTeX styles for use for Phys. Rev. journals
apsrmp4-1.bst     - BibTeX styles for use for Rev. Mod. Phys.
aipauth4-1.bst    - BibTeX styles for AIP journals with author/year style citations
aipnum4-1.bst     - BibTeX styles for AIP journals with numerical style citations


Documentation:       doc/latex/revtex/
                     -----------------
README       - How to get started
DOWNLOAD     - How to download REVTeX4.1

Author guide:           doc/latex/revtex/auguide/
                        ------
auguide4-1.tex (pdf)  - REVTeX 4.1 Author's Guide
whatsnew4-1.tex (pdf) - What's New in REVTeX 4.1
summary.tex (pdf)     - REVTeX 4.1 Command and Options Summary
docs.sty              - Package used by REVTeX documentation

APS guide:              doc/latex/revtex/aps
                        ------
apsguide4-1.tex (pdf) - APS Author Guide for REVTeX 4.1

AIP guide:              doc/latex/revtex/aip
                        ------
aipguide4-1.tex (pdf) - Author's Guide to AIP Substyles for REVTeX 4.1

APS Sample document:    doc/latex/revtex/sample/aps
                        -------
apssamp.tex (pdf)  - A sample file showing most common features of an APS
                     REVTeX 4.1 document
fig_1.eps          - sample figure for apssamp.tex
fig_2.eps          - sample wide figure for apssamp.tex
vid_1a.eps         - sample figure for apssamp.tex
vid_1b.eps         - sample figure for apssamp.tex
apssamp.bib        - sample BibTeX source file for apssamp.tex
apstemplate.tex    - A template for APS authors to follow

AIP Sample document:    doc/latex/revtex/sample/aip
                        -------
aipsamp.tex (pdf)  - A sample file showing most common features of an AIP
                     REVTeX 4.1 document
fig_1.eps          - sample figure for apssamp.tex
fig_2.eps          - sample wide figure for apssamp.tex
aipsamp.bib        - sample BibTeX source file for apssamp.tex
aiptemplate.tex    - A template for APS authors to follow


Programmer's docs:      doc/latex/revtex/source/
                        -------
ltxdocext.pdf - Programmer's documentation for the ltxdocext package
ltxfront.pdf  - Programmer's documentation for the ltxfront  package
ltxgrid.pdf   - Programmer's documentation for the ltxgrid   package
ltxutil.pdf   - Programmer's documentation for the ltxutil   package
revtex4-1.pdf - Programmer's documentation for the revtex4-1 document class
aip.pdf       - Programmer's documentation for the AIP journal styles

Source files:        source/latex/revtex
                     -------------------
ltxdocext.dtx - The source file for the ltxdocext package
ltxfront.dtx  - The source file for the ltxfront package
ltxgrid.dtx   - The source file for the ltxgrid package
ltxutil.dtx   - The source file for the ltxutil package
revtex4-1.dtx - The source file for revtex4.cls and revsymb.sty.
aip.dtx       - The source file for AIP journal styles

Not Included   
------------
The following packages are required by REVTeX but are not
included in this distribution. Please obtain from CTAN
(Comprehensive TeX Archive Network), e.g. <http://www.ctan.org/>. Direct
links to the necessary files can be found at <http://authors.aps.org/revtex4/>.

natbib.dtx   - Version 8.31a or later; found in latex/contrib/natbib on CTAN
natbib.ins   - LaTeX this to create natbib.sty and natbib
               documentation from natbib.dtx
bm.dtx       - Bold math style - part of (current!) standard LaTeX2e tools
bm.sty       - generated from bm.dtx by running tools.ins
textcase.dtx - Found in latex/contrib/textcase on CTAN
textcase.ins - LaTeX this to generate textcase.sty from textcase.dtx
url.sty      - Found in latex/contrib/misc on CTAN

An up-to-date installation of AMS-LaTeX is also required for certain
documentclass options. Version 2.0 or higher is needed. It is
available from <http://www.ams.org/tex/>.

Recommended styles and packages
--------------------------
With REVTeX implemented as a native LaTeX2e document class, users can 
take advantage of many of the well-supported LaTeX2e packages available.
Here are some that are particularly useful and recommended.

longtable.sty for tables running to multiple pages - part of a
standard LaTeX2e distribution.

hyperref.sty for hyperlinking - should work well with REVTeX 4.1.

graphics.sty and graphicx.sty for figure inclusion - part of LaTeX2e's
standard distribution.

Installation
------------
You already started the installation process by unzipping revtex4-1.zip.
As you will have seen, it created a directory revtex4.1 containing
this file README, the file DOWNLOAD, and the file revtex4-1-tds.zip, which
contains the bulk of the installation.

To install this software into a TDS-compliant TeX installation, like
TeX Live, working as root, issue a shell command like

  unzip revtex4-1-tds.zip -d /usr/local/texlive/texmf-local/
  
where the destination for the unzipped files is, in this example, 
appropriate for a local modificaton of a sufficiently recent distribution
of TeX Live. You may of course choose a different destination depending 
on your particular requirements. 

After installation, files will be located as per the Manifest above.

Run the appropriate update command (mktexlsr, initexmf -u, etc.); under
TeX Live that would be (as root)

   mktexlsr /usr/local/texlive/texmf-local

Install required packages (AMS-LaTeX, natbib, textcase, and bm). 
Please consult the documentaton for your local TeX package for more information. 
MikTeX users should use a recent version (see http://miktex.org/) and consult
the documentation there. There are several steps you will have to do. Please
note that the steps given here may change with future versions of MikTeX, but
the basic steps should be quite similar.
  1) Create a texmf-local directory if needed. For example, you might create
     a directory such as C:\local\miktex\texmf-local.
  2) Tell MikTeX where your texmf-local directory is. Find the MikTeX Options
     window and look for the "Roots" tab. If your texmf-local directory
     is not listed, click "Add" and add it.
  3) Unzip the revtex4-1-tds.zip (part of the REVTeX distribtution) in your
     texmf-local directory.
  4) Update the "File Name Database (FNDB)." This step is essential and
     it registers all of the files in your texmf-local directory with MikTeX.
     Do this by clicking on "Refresh FNDB" in the General tab of the MikTeX
     Options window.
     
MikTex also comes with a package manager. This can be an easier way to maintain
the packages installed on your system. However, please note that the packages
available may not be the most current version of the packages.

Credits
-------
David Carlisle created the first draft of REVTeX 4; Arthur Ogawa has 
supported the TeX development since. Patrick Daly was so kind as to 
incorporate needed changes into natbib and custom-bib. All worked under 
commission from the APS. Mark Doyle, APS Assistant Director, Journal
Information Systems coordinated the effort, which was partly underwritten
by the American Institute of Physics. The APS is the maintainer of REVTeX,
and all bugs are our responsibility. Please e-mail feedback to revtex@aps.org.

Backwards compatibility
-----------------------
The REVTeX 4.1 class file has been named revtex4-1.cls to distinguish it
from its predecessors. If the class file is copied to revtex4.cls,
files created with earlier versions of REVTeX 4 should still work.

LaTeX2e requirements
--------------------
REVTeX 4 requires: 
LaTeX2e [1996/06/01],
natbib  [2009/11/07]
textcase


==> revtex4-1/doc/latex/revtex/00readme.tex <==
\title{%
 The \classname{revtex4-1} document class of the American Physical Society%
 \protect\thanks{Work under hire to The American Physical Society.}%
}%
\author{Arthur Ogawa%
 \protect\thanks{First revision of REV\TeX4.0 (unreleased) by David Carlisle}%
}%
\date{Version \fileversion, dated \filedate}%
\newcommand\revtex{REV\TeX}

\maketitle

This file embodies the implementation of the APS \revtex\ 4.1 document class
for electronic submissions to journals.

The distribution point for this work is
\url{http://publish.aps.org/revtex4/},
which contains fully unpacked, prebuilt runtime files and documentation.

\tableofcontents

\section{Using \protect\revtex}

The file \file{README} has retrieval and installation information.

User documentation is presented separately in \file{auguide.tex}.

The file \file{template.aps} is a boilerplate file.

\changes{4.0a}{1998/01/16}{Initial version}
\changes{4.0a}{1998/01/31}{Move after process options, so \cs{clearpage} not in scope of twocolumn}
\changes{4.0a}{1998/01/31}{Rearrange the ordering so numerical ones come first. AO: David, what does this mean?}
\changes{4.0a}{1998/01/31}{use font-dependent spacing}
\changes{4.0a}{1998/01/31}{4.0d had twoside option setting twoside switch to false}
\changes{4.0a}{1998/01/31}{Move after process options, so the following test works}
\changes{4.0a}{1998/01/31}{print homepage}
\changes{4.0a}{1998/01/31}{protect against hyperref revtex kludges which are not needed now}
\changes{4.0a}{1998/06/10}{multiple preprint commands}
\changes{4.0a}{1998/06/10}{comma not space between email and homepage}
\changes{4.0a}{1998/06/10}{single space footnotes}
\changes{4.0b}{1999/06/20}{First modifications by Arthur Ogawa (mailto:arthur\_ogawa at sbcglobal dot net)}
\changes{4.0b}{1999/06/20}{Added localization of \cs{figuresname}}
\changes{4.0b}{1999/06/20}{Added localization of \cs{tablesname}}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{10pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{11pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: all code for \protect\classoption{12pt} is in this module.}
\changes{4.0b}{1999/06/20}{AO: made aps.rtx part of revtex4.dtx}
\changes{4.0b}{1999/06/20}{AO: remove duplicates}
\changes{4.0b}{1999/06/20}{call \cs{print@floats}}
\changes{4.0b}{1999/06/20}{Defer assignment until \cs{AtBeginDocument} time.}
\changes{4.0b}{1999/06/20}{Defer decision until \cs{AtBeginDocument} time}
\changes{4.0b}{1999/06/20}{Define three separate environments, defer assignment to \cs{AtBeginDocument} time.}
\changes{4.0b}{1999/06/20}{Frank Mittelbach, has stated in \protect\classname{multicol}: ``The kernel command \cs{@footnotetext} should not be modified.'' Thus, I have removed David Carlisle's redefinition of that command. Note, however, that later versions of \protect\classname{multicol} do not require this workaround. Belt and suspenders.}%
\changes{4.0b}{1999/06/20}{Move this ``complex'' option to the front, where it can be overridden by ``simple'' options.}
\changes{4.0b}{1999/06/20}{New option}
\changes{4.0b}{1999/06/20}{One-line caption sets flush left.}
\changes{4.0b}{1999/06/20}{only execute if appropriate}
\changes{4.0b}{1999/06/20}{Processing delayed to \cs{AtBeginDocument} time}
\changes{4.0b}{1999/06/20}{Removed invocation of nonexistent class option \protect\classoption{groupauthors} and all other class options that should only be invoked by the document. (Otherwise precedence of class options does not work.)}
\changes{4.0b}{1999/06/20}{Restore all media size class option of \protect\file{classes.dtx}}
\changes{4.0b}{1999/06/20}{Stack \cs{preprint} args flush right at right margin.}
\changes{4.0c}{1999/11/13}{(AO, 115) If three or more preprints specified, set on single line, with commas.}
\changes{4.0c}{1999/11/13}{(AO, 129) section* within appendix was producing appendixname}
\changes{4.0c}{1999/11/13}{*-form mandates pagebreak}
\changes{4.0c}{1999/11/13}{also spelled ``acknowledgements''.}
\changes{4.0c}{1999/11/13}{Do not put by REVTeX in every page foot}
\changes{4.0c}{1999/11/13}{grid changes via ltxgrid procedures}
\changes{4.0c}{1999/11/13}{grid changes with ltxgrid}
\changes{4.0c}{1999/11/13}{Insert procedure \cs{checkindate}}
\changes{4.0c}{1999/11/13}{Lose compatability mode.}
\changes{4.0c}{1999/11/13}{New ltxgrid-based  code, other bug fixes}
\changes{4.0c}{1999/11/13}{New option ``checkin''}
\changes{4.0c}{1999/11/13}{Prevent an inner footnote from performing twice}
\changes{4.0d}{2000/04/10}{Also alter how lists get indented.}
\changes{4.0d}{2000/04/10}{eprint takes an optional argument, syntactical only in this case.}
\changes{4.0d}{2000/04/10}{New option}
\changes{4.0d}{2000/05/10}{More features and bug fixes: compatability with longtable and array packages. Now certainly incompatible with multicol.}
\changes{4.0d}{2000/05/17}{make longtable trigger the head, too}
\changes{4.0d}{2000/05/18}{But alternative spelling is deprecated.}
\changes{4.0e}{2000/09/20}{New option showkeys}
\changes{4.0e}{2000/11/14}{Bug fixes and minor new features: title block affiliations can have ancillary data, just like authors; clearpage processing revamped, with floats staying in order; widetext ornaments.}
\changes{4.0e}{2000/11/21}{adornments above and below.}
\changes{4.0f}{2001/02/13}{Last bug fixes before release.}
\changes{4.0rc1}{2001/06/17}{Running headers always as if two-sided}
\changes{4.0rc1}{2001/06/18}{grid changes with push and pop}
\changes{4.0rc1}{2001/06/18}{grid changes with push and pop}
\changes{4.0rc4}{2001/07/23}{hyperref is no longer loaded via class option: use a usepackage statement instead}
\changes{4.1a}{2008/01/18}{(AO, 457) Endnotes to be sorted in with numerical citations.}%
\changes{4.1a}{2008/01/18}{(AO, 451) ``Cannot have more than 256 cites in a document''}%
\changes{4.1a}{2008/01/18}{(AO, 457) Endnotes to be sorted in with numerical citations.}%
\changes{4.1a}{2008/01/18}{(AO, 460) ``Proper style is "FIG. 1. ..." (no colon)''}%
\changes{4.1a}{2008/01/18}{(AO, 478) \cs{ds@letterpaper}, so that ``letterpaper really is the default''}%
\changes{4.1a}{2008/01/18}{(AO, 488) Change processing of options to allow an unused option to specify society and journal}%
\changes{4.1a}{2008/01/19}{(AO, 461) Change the csname revtex uses from @dotsep to ltxu@dotsep. The former is understood in mu. (What we wanted was a dimension.)}%
\changes{4.1a}{2008/01/19}{For natbib versions before 8.21, \cs{NAT@sort} was consulted only as natbib was being read in. Now it is fully dynamic.}
\changes{4.1b}{2008/05/29}{The csname substyle@ext is now defined without a dot (.), to be compatible with \LaTeX usage (see @clsextension and @pkgextension).}
\changes{4.1b}{2008/06/01}{(AO) Implement bibnotes through \cs{frontmatter@footnote@produce} instead of \cs{bibnotes@sw}}%
\changes{4.1b}{2008/06/01}{Add option reprint, opposite of preprint, and preferred alternative to twocolumn}
\changes{4.1b}{2008/06/29}{(AO, 455) Be nice to a list within the abstract (assign \cs{@totalleftmargin}).}
\changes{4.1b}{2008/06/30}{(AO) Structure the Abstract using the \texttt{bibliography} environment}
\changes{4.1b}{2008/07/01}{(AO) coordinate \cs{if@twoside} with \cs{twoside@sw}}
\changes{4.1b}{2008/07/01}{(AO) make settings at class time instead of deferring them to later.}
\changes{4.1b}{2008/07/01}{(AO) No longer need to test \cs{chapter} as of \texttt{natbib} version 8.2}
\changes{4.1b}{2008/07/01}{(AO) No longer use \cs{secnumarabic@sw}, instead use \cs{setup@secnums}}
\changes{4.1b}{2008/07/01}{(AO) Provide more diagnostics when \cs{@society} is assigned.}
\changes{4.1b}{2008/07/01}{(AO) provide option longbibliography}
\changes{4.1b}{2008/07/01}{Add \cs{@hangfroms@section}}
\changes{4.1b}{2008/07/01}{Break out \cs{@caption@fignum@sep}}
\changes{4.1b}{2008/07/01}{Class option galley sets \cs{preprintsty@sw} to false}
\changes{4.1b}{2008/07/01}{Code relating to new syntax for frontmatter has been placed in \file{ltxfront.dtx}}
\changes{4.1b}{2008/07/01}{Package textcase is now simply a required package}
\changes{4.1b}{2008/07/01}{Procedures \cs{@parse@class@options@society} and \cs{@parse@class@options@journal} and friends}
\changes{4.1b}{2008/07/01}{Read in all required packages together}
\changes{4.1b}{2008/07/01}{Remove options newabstract and oldabstract}
\changes{4.1b}{2008/08/01}{Section numbering via procedures \cs{secnums@rtx} and \cs{secnums@arabic}.}
\changes{4.1b}{2008/08/04}{As with author formatting, rag the right more, and assign \cs{@totalleftmargin}. Also neutralize \cs{def@after@address}.}%
\changes{4.1b}{2008/08/04}{Rag the right even more: .8\cs{hsize}. Also, assign \cs{@totalleftmargin}.}%
\changes{4.1b}{2008/08/04}{The \texttt{rmp} journal substyle selects \texttt{groupedaddress} by default.}%
\changes{4.1b}{2008/08/04}{Use \cs{setup@hook} to initialize all.}
\changes{4.1c}{2008/08/15}{Document class option longbibliography via \cs{substyle@post}}
\changes{4.1d}{2009/03/27}{Definition of \cs{ @fnsymbol} follows fixltx2e.sty}
\changes{4.1e}{2008/06/29}{(AO, 455) be nice to a list within the abstract}
\changes{4.1f}{2009/07/07}{(AO, 513) Add class option linenumbers: number the lines a la \classname{lineno}}
\changes{4.1f}{2009/07/07}{(AO, 516) Merged references are separated with a semicolon}
\changes{4.1f}{2009/07/10}{(AO, 520) Automatically produce \cs{bibliography} command when needed}%
\changes{4.1f}{2009/07/11}{(AO, 521) Lonely bibliography head}%
\changes{4.1f}{2009/07/11}{(AO, 522) Warn if software is expired}%
\changes{4.1f}{2009/07/15}{(AO, 523) Add class option nomerge, to turn off new natbib 8.3 syntax}
\changes{4.1f}{2009/07/20}{(AO, 524) Makes no sense if citations are superscript numbers and so are footnotes}
\changes{4.1f}{2009/10/05}{(AO, 530) \cs{@fnsymbol}: Failed to import fixltx2e.sty technology. Return to LaTeX core.}
\changes{4.1g}{2009/10/07}{(AO, 525) Remove phantom paragraph above display math that is given in vertical mode}%
\changes{4.1g}{2009/10/07}{(AO, 538) \cs{MakeTextUppercase} inappropriately expands the double backslash}
\changes{4.1h}{2009/10/09}{(AO) Remove expiry code in the release software}%
\changes{4.1i}{2009/10/23}{(AO, 541) Defer assignment of \cs{cite} until after natbib loads}
\changes{4.1j}{2009/10/24}{(AO, 549) Repairing natbib's \cs{BibitemShut} and \cs{bibAnnote}}
\changes{4.1j}{2009/10/25}{(AO, 545) hypertext capabilities off by default; enable with \classoption{hypertext}}
\changes{4.1j}{2009/10/25}{(AO, 552) Repair spacing in \cs{onlinecite}}
\changes{4.1k}{2009/11/06}{(AO, 554) give the \cs{newlabel} command syntax appropriate to the hyperref package}
\changes{4.1n}{2009/11/06}{(AO, 565) restore 4.0 behavior: invoking class option preprint implies class option preprintnumbers}
\changes{4.1n}{2009/11/30}{(AO, 566) restore 4.0 behavior: flush column bottoms}
\changes{4.1n}{2009/12/05}{(AO, 569) Use of \classname{hyperref} interferes with column balancing of last page}%
\changes{4.1n}{2009/12/09}{(AO, 569) execute the after-last-shipout procedures from within the safety of the output routine}%
\changes{4.1n}{2010/01/02}{(AO, 571) Interface \cs{set@footnotewidth} for determining the set width of footnotes}%
\changes{4.1n}{2010/01/02}{(AO, 572) Independent footnote counter for title block. Abstract footnote counter shared with body.}%
\changes{4.1n}{2009/12/13}{(AO, 573) arrange to load \classname{lineno} after any other packages.}%
\changes{4.1n}{2010/01/04}{(AO, 575) the default for journal prstper is longbibliography}%
\changes{4.1n}{2010/01/04}{(AO, 576) In .bst files, remove support for the annote field}%
\changes{4.1n}{2010/01/02}{(AO) fine-tune spacing above and below widetext}%
\changes{4.1n}{2010/01/02}{(AO, 571) class file must set \cs{splittopskip}; fine tune \cs{skip}\cs{footins}; \cs{footnoterule} defined in terms of \cs{skip}\cs{footins}}%
\changes{4.1n}{2010/01/02}{(AO, 572) \cs{@makefntext} and \cs{frontmatter@makefntext} must be defined harmoniously}%
\changes{4.1o}{2010/02/02}{(AO, 575) Automatically incorporate the (Bib\TeX-generated) .bbl into an explicit \env{thebibliography}}%
\changes{4.1o}{2010/02/05}{(AO, 549) Remove patch to natbib, which is now at version 8.31a}
\changes{4.1o}{2010/02/07}{(AO, 578) accommodate the possible space character preceding \cs{BibitemShut}.}
\changes{4.1o}{2010/02/05}{(AO, 579) Endnote shall comprise their own Bib\TeX\ entry type: @FOOTNOTE.}
\changes{4.1o}{2010/02/10}{(AO, 580) Provide a document class option to turn off production of eprint field in bibliography.}
\changes{4.1o}{2010/02/12}{(AO, 580) Control .bst at run time.}%
\changes{4.1o}{2010/02/09}{(AO, 581) Handle case: merged references, with first ending in a stop character.}
\changes{4.1p}{2010/02/24}{(AO, 583) Provide interface to \classname{ltxgrid} \cs{onecolumn@grid@setup} and \cs{twocolumn@grid@setup}}
\changes{4.1p}{2010/02/24}{(AO, 584) Per MD, remove trailing space character from each journal abbreviation: it had caused an extraneous space in the .bbl}
\changes{4.1q}{2010/04/01}{(AO, 586) When .bbl is pasted into the document, prevent automatic bibliography inclusion.}%
\changes{4.1q}{2010/04/13}{(AO, 588) Only write \revtex-specific BibTeX .bib data if the .bst style is set by REVTeX.}%
\changes{4.1r}{2010/06/22}{(AO, 595) Provide \cs{lovname} along with other List of Videos definitions.}%

\iffalse ltxdoc klootch
This file has version number 4.1r, last revised 2010/07/25/20:33:00.\fi


==> revtex4-1/doc/latex/revtex/README <==
%% ****** Start of file README ****** %
%%
%%   This file is part of the APS files in the REVTeX 4 distribution.
%%   Version 4.1r of REVTeX, August 2010.
%%
%%   Copyright (c) 1999, 2000, 2001, 2009, 2010 The American Physical Society.
%%

Last updated 09 August 2010

This file describes the contents of this distribution of REVTeX 4.1.
The definitive source of information about REVTeX 4 is the APS web
page http://authors.aps.org/revtex4/.

User queries should be directed to revtex@aps.org.

Manifest
--------

All files in this release are contained within the compressed archive
revtex4-1.zip. For installation instructions, see below.

NOTE: The only files necessary for running REVTeX 4.1 are those under 
tex/latex/revtex and bibtex/bst/revtex, but it is a good idea to install
the entire distribution, especially the documentation.

TeX inputs:          tex/latex/revtex/
                     -----------------  
revtex4-1.cls     - The REVTeX 4.1 class file
aps4-1.rtx        - APS-specific customizations for REVTeX 4.1
aip4-1.rtx        - AIP-specific customizations for REVTeX 4.1
apsrmp4-1.rtx     - APS-specific customizations for REVTeX 4.1,
                    specifically for Rev. Mod. Phys.
aps10pt4-1.rtx    - 10-point size class option file for REVTeX.
aps11pt4-1.rtx    - 11-point size class option file for REVTeX.
aps12pt4-1.rtx    - 12-point size class option file for REVTeX.
revsymb4-1.sty    - A collection of common symbols for use outside of REVTeX.

ltxdocext.sty     - Part of ltxgrid package used for page layout in REVTeX.
ltxfront.sty      - Part of ltxgrid package used for page layout in REVTeX.
ltxgrid.sty       - Part of ltxgrid package used for page layout in REVTeX.
ltxutil.sty       - Part of ltxgrid package used for page layout in REVTeX.
  
BibTeX inputs:       bibtex/bst/revtex/
                     ------------------ 
apsrev4-1.bst     - BibTeX styles for use for Phys. Rev. journals
apsrmp4-1.bst     - BibTeX styles for use for Rev. Mod. Phys.
aipauth4-1.bst    - BibTeX styles for AIP journals with author/year style citations
aipnum4-1.bst     - BibTeX styles for AIP journals with numerical style citations


Documentation:       doc/latex/revtex/
                     -----------------
README       - How to get started
DOWNLOAD     - How to download REVTeX4.1

Author guide:           doc/latex/revtex/auguide/
                        ------
auguide4-1.tex (pdf)  - REVTeX 4.1 Author's Guide
whatsnew4-1.tex (pdf) - What's New in REVTeX 4.1
summary.tex (pdf)     - REVTeX 4.1 Command and Options Summary
docs.sty              - Package used by REVTeX documentation

APS guide:              doc/latex/revtex/aps
                        ------
apsguide4-1.tex (pdf) - APS Author Guide for REVTeX 4.1

AIP guide:              doc/latex/revtex/aip
                        ------
aipguide4-1.tex (pdf) - Author's Guide to AIP Substyles for REVTeX 4.1

APS Sample document:    doc/latex/revtex/sample/aps
                        -------
apssamp.tex (pdf)  - A sample file showing most common features of an APS
                     REVTeX 4.1 document
fig_1.eps          - sample figure for apssamp.tex
fig_2.eps          - sample wide figure for apssamp.tex
vid_1a.eps         - sample figure for apssamp.tex
vid_1b.eps         - sample figure for apssamp.tex
apssamp.bib        - sample BibTeX source file for apssamp.tex
apstemplate.tex    - A template for APS authors to follow

AIP Sample document:    doc/latex/revtex/sample/aip
                        -------
aipsamp.tex (pdf)  - A sample file showing most common features of an AIP
                     REVTeX 4.1 document
fig_1.eps          - sample figure for apssamp.tex
fig_2.eps          - sample wide figure for apssamp.tex
aipsamp.bib        - sample BibTeX source file for apssamp.tex
aiptemplate.tex    - A template for APS authors to follow


Programmer's docs:      doc/latex/revtex/source/
                        -------
ltxdocext.pdf - Programmer's documentation for the ltxdocext package
ltxfront.pdf  - Programmer's documentation for the ltxfront  package
ltxgrid.pdf   - Programmer's documentation for the ltxgrid   package
ltxutil.pdf   - Programmer's documentation for the ltxutil   package
revtex4-1.pdf - Programmer's documentation for the revtex4-1 document class
aip.pdf       - Programmer's documentation for the AIP journal styles

Source files:        source/latex/revtex
                     -------------------
ltxdocext.dtx - The source file for the ltxdocext package
ltxfront.dtx  - The source file for the ltxfront package
ltxgrid.dtx   - The source file for the ltxgrid package
ltxutil.dtx   - The source file for the ltxutil package
revtex4-1.dtx - The source file for revtex4.cls and revsymb.sty.
aip.dtx       - The source file for AIP journal styles

Not Included   
------------
The following packages are required by REVTeX but are not
included in this distribution. Please obtain from CTAN
(Comprehensive TeX Archive Network), e.g. <http://www.ctan.org/>. Direct
links to the necessary files can be found at <http://authors.aps.org/revtex4/>.

natbib.dtx   - Version 8.31a or later; found in latex/contrib/natbib on CTAN
natbib.ins   - LaTeX this to create natbib.sty and natbib
               documentation from natbib.dtx
bm.dtx       - Bold math style - part of (current!) standard LaTeX2e tools
bm.sty       - generated from bm.dtx by running tools.ins
textcase.dtx - Found in latex/contrib/textcase on CTAN
textcase.ins - LaTeX this to generate textcase.sty from textcase.dtx
url.sty      - Found in latex/contrib/misc on CTAN

An up-to-date installation of AMS-LaTeX is also required for certain
documentclass options. Version 2.0 or higher is needed. It is
available from <http://www.ams.org/tex/>.

Recommended styles and packages
--------------------------
With REVTeX implemented as a native LaTeX2e document class, users can 
take advantage of many of the well-supported LaTeX2e packages available.
Here are some that are particularly useful and recommended.

longtable.sty for tables running to multiple pages - part of a
standard LaTeX2e distribution.

hyperref.sty for hyperlinking - should work well with REVTeX 4.1.

graphics.sty and graphicx.sty for figure inclusion - part of LaTeX2e's
standard distribution.

Installation
------------
You already started the installation process by unzipping revtex4-1.zip.
As you will have seen, it created a directory revtex4.1 containing
this file README, the file DOWNLOAD, and the file revtex4-1-tds.zip, which
contains the bulk of the installation.

To install this software into a TDS-compliant TeX installation, like
TeX Live, working as root, issue a shell command like

  unzip revtex4-1-tds.zip -d /usr/local/texlive/texmf-local/
  
where the destination for the unzipped files is, in this example, 
appropriate for a local modificaton of a sufficiently recent distribution
of TeX Live. You may of course choose a different destination depending 
on your particular requirements. 

After installation, files will be located as per the Manifest above.

Run the appropriate update command (mktexlsr, initexmf -u, etc.); under
TeX Live that would be (as root)

   mktexlsr /usr/local/texlive/texmf-local

Install required packages (AMS-LaTeX, natbib, textcase, and bm). 
Please consult the documentaton for your local TeX package for more information. 
MikTeX users should use a recent version (see http://miktex.org/) and consult
the documentation there. There are several steps you will have to do. Please
note that the steps given here may change with future versions of MikTeX, but
the basic steps should be quite similar.
  1) Create a texmf-local directory if needed. For example, you might create
     a directory such as C:\local\miktex\texmf-local.
  2) Tell MikTeX where your texmf-local directory is. Find the MikTeX Options
     window and look for the "Roots" tab. If your texmf-local directory
     is not listed, click "Add" and add it.
  3) Unzip the revtex4-1-tds.zip (part of the REVTeX distribtution) in your
     texmf-local directory.
  4) Update the "File Name Database (FNDB)." This step is essential and
     it registers all of the files in your texmf-local directory with MikTeX.
     Do this by clicking on "Refresh FNDB" in the General tab of the MikTeX
     Options window.
     
MikTex also comes with a package manager. This can be an easier way to maintain
the packages installed on your system. However, please note that the packages
available may not be the most current version of the packages.

Credits
-------
David Carlisle created the first draft of REVTeX 4; Arthur Ogawa has 
supported the TeX development since. Patrick Daly was so kind as to 
incorporate needed changes into natbib and custom-bib. All worked under 
commission from the APS. Mark Doyle, APS Assistant Director, Journal
Information Systems coordinated the effort, which was partly underwritten
by the American Institute of Physics. The APS is the maintainer of REVTeX,
and all bugs are our responsibility. Please e-mail feedback to revtex@aps.org.

Backwards compatibility
-----------------------
The REVTeX 4.1 class file has been named revtex4-1.cls to distinguish it
from its predecessors. If the class file is copied to revtex4.cls,
files created with earlier versions of REVTeX 4 should still work.

LaTeX2e requirements
--------------------
REVTeX 4 requires: 
LaTeX2e [1996/06/01],
natbib  [2009/11/07]
textcase

